Leveraging Siamese Networks for One-Shot Intrusion Detection Model

The use of supervised Machine Learning (ML) to enhance Intrusion Detection Systems has been the subject of significant research. Supervised ML is based upon learning by example, demanding significant volumes of representative instances for effective training and the need to re-train the model for every unseen cyber-attack class. However, retraining the models in-situ renders the network susceptible to attacks owing to the time-window required to acquire a sufficient volume of data. Although anomaly detection systems provide a coarse-grained defence against unseen attacks, these approaches are significantly less accurate and suffer from high false-positive rates. Here, a complementary approach referred to as 'One-Shot Learning', whereby a limited number of examples of a new attack-class is used to identify a new attack-class (out of many) is detailed. The model grants a new cyber-attack classification without retraining. A Siamese Network is trained to differentiate between classes based on pairs similarities, rather than features, allowing to identify new and previously unseen attacks. The performance of a pre-trained model to classify attack-classes based only on one example is evaluated using three datasets. Results confirm the adaptability of the model in classifying unseen attacks and the trade-off between performance and the need for distinctive class representation.

==> extra-tables.tex <==
\section{}
\setcounter{table}{0}
\renewcommand{\thetable}{A.\arabic{table}}
%\subsection*{One-Shot (CICIDS)}
\input{result-tables/one-shot/cicids-hulk-one-shot.tex}
\input{result-tables/one-shot/cicids-slowloris-one-shot.tex}


%\subsection*{One-Shot (NSL-KDD)}
\input{result-tables/one-shot/nsl-kdd-probe.tex}
\input{result-tables/one-shot/nsl-kdd-r2l.tex}
\input{result-tables/one-shot/nsl-kdd-u2r.tex}

%\subsection*{One-Shot (KDD Cup'99)}
\input{result-tables/one-shot/kdd-probe.tex}
\input{result-tables/one-shot/kdd-r2l.tex}
\input{result-tables/one-shot/kdd-u2r.tex}

%\subsection*{Zero-Day (KDD Cup'99)}
% \input{result-tables/zero-day/kdd-dos.tex}
% \input{result-tables/zero-day/kdd-probe.tex}
% \input{result-tables/zero-day/kdd-u2r.tex}

%\subsection*{Zero-Day (NSL-KDD)}
% \input{result-tables/zero-day/nsl-kdd-dos.tex}
% \input{result-tables/zero-day/nsl-kdd-probe.tex}
% \input{result-tables/zero-day/nsl-kdd-u2r.tex}

%\subsection*{One-Shot (SCADA)}
% \input{result-tables/one-shot/scada-blocked1.tex}
% \input{result-tables/one-shot/scada-blocked2.tex}
% \input{result-tables/one-shot/scada-hum.tex}
% \input{result-tables/one-shot/scada-2.tex}
% \input{result-tables/one-shot/scada-7.tex}
% \input{result-tables/one-shot/scada-high.tex}
% \input{result-tables/one-shot/scada-med.tex}
% \input{result-tables/one-shot/scada-low.tex}
% \input{result-tables/one-shot/scada-plastic.tex}
% \input{result-tables/one-shot/scada-sensor.tex}
% \input{result-tables/one-shot/scada-spoofing.tex}
% \input{result-tables/one-shot/scada-wrong.tex}


%\subsection*{Zero-Day (SCADA)}
% \input{result-tables/zero-day/scada-blocked1.tex}
% \input{result-tables/zero-day/scada-blocked2.tex}
% \input{result-tables/zero-day/scada-hum.tex}
% \input{result-tables/zero-day/scada-2.tex}
% \input{result-tables/zero-day/scada-7.tex}
% \input{result-tables/zero-day/scada-high.tex}
% \input{result-tables/zero-day/scada-med.tex}
% \input{result-tables/zero-day/scada-low.tex}
% \input{result-tables/zero-day/scada-plastic.tex}
% \input{result-tables/zero-day/scada-sensor.tex}
% \input{result-tables/zero-day/scada-spoofing.tex}
% \input{result-tables/zero-day/scada-wrong.tex}

% \section{}
% \label{apx:cic2}
% \hl{To further evaluate the proposed model, another set of experiments were conducted using a different set of CICIDS2017 classes. The same evaluation method using the same proposed model in Section~\ref{sec:one-shot} is performed. The used classes are listed in Table~\ref{tab:cicattacks_2}. }

% \begin{table}[thb]
%     \centering
%     \caption{\hl{CICIDS Classes and Corresponding Number of Occurrences (2)}}
%     \begin{tabular}{|c|c|c|}
%          \hline
%          \rowcolor{gray!30}
%          & Class & \# of Occurrences\\ \hline
%          1 & Normal & 248607 (53.47\%) \\ \hline
%          2 & Port Scan & 165252 (35.55\%) \\ \hline
%          3 & DDoS & 45523 (9.79\%) \\ \hline
%          4 & Heartbleed & 346 (0.07\%) \\ \hline
%          5 & FTP Brute Force & 5228 (1.12\%) \\ \hline
%     \end{tabular}
%     \label{tab:cicattacks_2}
% \end{table}


% The performance evaluation results are listed as follows; excluding the Heartbleed class from the training results are presented in Table~\ref{tab:cicids2-heartbleed-one-shot} and Table~\ref{tab:cicids2-heartbleed-one-shot-pairs}, DDoS in Table~\ref{tab:cicids2-ddos-one-shot} and Table~\ref{tab:cicids2-ddos-one-shot-pairs}, the Port Scan results are presented in Table~\ref{tab:cicids2-portscan-one-shot} and Table~\ref{tab:cicids2-portscan-one-shot-pairs}, while the FTP Brute Force in Table~\ref{tab:cicids2-ftp-one-shot} and Table~\ref{tab:cicids2-ftp-one-shot-pairs}.


% \input{result-tables/one-shot/cicids2_heartbleed}
% \input{result-tables/one-shot/cicids2_ddos}
% \input{result-tables/one-shot/cicids2_portscan}
% \input{result-tables/one-shot/cicids2_ftp}


==> result-tables/one-shot/cicids2_ddos.tex <==
\begin{table}[h]
    \centering
    \caption{CICIDS2017 One-Shot Confusion Matrix (DDoS Not in Training)}
    \begin{tabular}{|C{0.15\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\columnwidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.1\NetTableWidth}|}
    \hhline{~-----~}
    \multicolumn{1}{c|}{} &
    \multicolumn{5}{c|}{\cellcolor{tabhead}Predicted Class} & \multicolumn{1}{|c}{}  \\
    \hline
    \rowcolor{tabhead}
     Correct &  Normal & Heart-bleed & DDoS & Port Scan & FTP & Overall \\ \hline
    \cellcolor{tabhead}Normal & 3812 \newline \cellcolor{tabhead}\textbf{(63.53\%)} & 605 \newline \textit{(10.08\%)} & 1455 \newline \textit{(24.25\%)} & 72 \newline \textit{(1.2\%)} & 56 \newline \textit{(0.93\%)} & \multirow{5}{*}{80.36\%}\\ \cline{1-6}
    \cellcolor{tabhead}Heartbleed & 1376 \newline \textit{(22.93\%)} & 4070 \newline \cellcolor{tabhead}\textbf{(67.83\%)} & 33 \newline \textit{(0.55\%)} & 79 \newline \textit{(1.32\%)} & 442 \newline \textit{(7.37\%)} & \\ \cline{1-6}
    \cellcolor{classcol}DDoS & 243 \newline \textit{(4.05\%)} & 85 \newline \textit{(1.42\%)} & 5646 \newline \cellcolor{classcol}\textbf{(94.1\%)} & 14 \newline \textit{(0.23\%)} & 12 \newline \textit{(0.2\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}Port Scan & 62 \newline \textit{(1.03\%)} & 83 \newline \textit{(1.38\%)} & 6 \newline \textit{(0.1\%)} & 5832 \newline \cellcolor{tabhead}\textbf{(97.2\%)} & 17 \newline \textit{(0.28\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}FTP & 410 \newline \textit{(6.83\%)} & 808 \newline \textit{(13.47\%)} & 13 \newline \textit{(0.22\%)} & 21 \newline \textit{(0.35\%)} & 4748 \newline \cellcolor{tabhead}\textbf{(79.13\%)} & \\ \hline
    \end{tabular}

    \label{tab:cicids2-ddos-one-shot}
\end{table}


\begin{table}[H]
    \caption{CICIDS2017 One-Shot Accuracy (DDoS not in Training) Using Different $j$ Votes}
    \centering
    \begin{tabular}{|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|}
        \hline
        \rowcolor{tabhead}
         No Votes & Overall & \multicolumn{2}{c|}{New Class (DDoS)} &  \multicolumn{2}{c|}{Normal} \\ \cline{3-6} 
        \rowcolor{tabhead}
        ($j$) & Accuracy&  TPR & FNR & TNR & FPR \\  \hline
        \cellcolor{tabhead}1&73.42\% &87.72\% &10.18\% &53.9\% &46.1\%\\ \hline
        \cellcolor{tabhead}5&80.36\% &94.1\% &4.05\% &63.53\% &36.47\%\\ \hline
        \cellcolor{tabhead}10&82.38\% &94.77\% &3.35\% &69.1\% &30.9\%\\ \hline
        \cellcolor{tabhead}15&82.17\% &96.65\% &1.47\% &65.97\% &34.03\%\\ \hline
        \cellcolor{tabhead}20&82.75\% &96.98\% &1.13\% &68.42\% &31.58\%\\ \hline
        \cellcolor{tabhead}25&82.27\% &97.48\% &0.63\% &65.63\% &34.37\%\\ \hline
        \cellcolor{tabhead}30&82.53\% &97.52\% &0.6\% &67.13\% &32.87\%\\ \hline
     \hline 

    \end{tabular}
    
    \label{tab:cicids2-ddos-one-shot-pairs}
    
\end{table}


==> result-tables/one-shot/cicids2_ftp.tex <==
\begin{table}[h]
    \centering
    \caption{CICIDS2017 One-Shot Confusion Matrix (FTP Not in Training)}
    \begin{tabular}{|C{0.15\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\columnwidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.1\NetTableWidth}|}
    \hhline{~-----~}
    \multicolumn{1}{c|}{} &
    \multicolumn{5}{c|}{\cellcolor{tabhead}Predicted Class} & \multicolumn{1}{|c}{}  \\
    \hline
    \rowcolor{tabhead}
     Correct &  Normal & Heart-bleed & DDoS & Port Scan & FTP & Overall \\ \hline
    \cellcolor{tabhead}Normal & 5120 \newline \cellcolor{tabhead}\textbf{(85.33\%)} & 784 \newline \textit{(13.07\%)} & 40 \newline \textit{(0.67\%)} & 3 \newline \textit{(0.05\%)} & 53 \newline \textit{(0.88\%)} & \multirow{5}{*}{83.14\%}\\ \cline{1-6}
    \cellcolor{tabhead}Heartbleed & 1696 \newline \textit{(28.27\%)} & 4049 \newline \cellcolor{tabhead}\textbf{(67.48\%)} & 63 \newline \textit{(1.05\%)} & 15 \newline \textit{(0.25\%)} & 177 \newline \textit{(2.95\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}DDoS & 61 \newline \textit{(1.02\%)} & 36 \newline \textit{(0.6\%)} & 5892 \newline \cellcolor{tabhead}\textbf{(98.2\%)} & 2 \newline \textit{(0.03\%)} & 9 \newline \textit{(0.15\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}Port Scan & 50 \newline \textit{(0.83\%)} & 94 \newline \textit{(1.57\%)} & 6 \newline \textit{(0.1\%)} & 5817 \newline \cellcolor{tabhead}\textbf{(96.95\%)} & 33 \newline \textit{(0.55\%)} & \\ \cline{1-6}
    \cellcolor{classcol}FTP & 485 \newline \textit{(8.08\%)} & 807 \newline \textit{(13.45\%)} & 24 \newline \textit{(0.4\%)} & 621 \newline \textit{(10.35\%)} & 4063 \newline \cellcolor{classcol}\textbf{(67.72\%)} & \\ \hline
    \end{tabular}

    \label{tab:cicids2-ftp-one-shot}
\end{table}


\begin{table}[H]
    \caption{CICIDS2017 One-Shot Accuracy (FTP not in Training) Using Different $j$ Votes}
    \centering
    \begin{tabular}{|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|}
        \hline
        \rowcolor{tabhead}
         No Votes & Overall & \multicolumn{2}{c|}{New Class (FTP)} &  \multicolumn{2}{c|}{Normal} \\ \cline{3-6} 
        \rowcolor{tabhead}
        ($j$) & Accuracy&  TPR & FNR & TNR & FPR \\  \hline
        \cellcolor{tabhead}1&75.52\% &58.05\% &7.37\% &70.53\% &29.47\%\\ \hline
        \cellcolor{tabhead}5&83.14\% &67.72\% &8.08\% &85.33\% &14.67\%\\ \hline
        \cellcolor{tabhead}10&84.3\% &69.75\% &8.07\% &87.02\% &12.98\%\\ \hline
        \cellcolor{tabhead}15&85.61\% &75.18\% &8.05\% &87.73\% &12.27\%\\ \hline
        \cellcolor{tabhead}20&85.7\% &75.55\% &8.08\% &87.98\% &12.02\%\\ \hline
        \cellcolor{tabhead}25&85.95\% &76.72\% &8.22\% &87.98\% &12.02\%\\ \hline
        \cellcolor{tabhead}30&86.01\% &76.98\% &8.17\% &87.97\% &12.03\%\\ \hline



     \hline 

    \end{tabular}
    
    \label{tab:cicids2-ftp-one-shot-pairs}
    
\end{table}


==> result-tables/one-shot/cicids2_heartbleed.tex <==
\begin{table}[h]
    \centering
    \caption{CICIDS2017 One-Shot Confusion Matrix (Heartbleed Not in Training)}
    \begin{tabular}{|C{0.15\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\columnwidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.1\NetTableWidth}|}
    \hhline{~-----~}
    \multicolumn{1}{c|}{} &
    \multicolumn{5}{c|}{\cellcolor{tabhead}Predicted Class} & \multicolumn{1}{|c}{}  \\
    \hline
    \rowcolor{tabhead}
     Correct &  Normal & Heart-bleed & DDoS & Port Scan & FTP & Overall \\ \hline
    \cellcolor{tabhead}Normal & 4467 \newline \cellcolor{tabhead}\textbf{(74.45\%)} & 1355 \newline \textit{(22.58\%)} & 49 \newline \textit{(0.82\%)} & 44 \newline \textit{(0.73\%)} & 85 \newline \textit{(1.42\%)} & \multirow{5}{*}{82.7\%}\\ \cline{1-6}
    \cellcolor{classcol}Heartbleed & 1918 \newline \textit{(31.97\%)} & 3893 \newline \cellcolor{classcol}\textbf{(64.88\%)} & 0 \newline \textit{(0\%)} & 1 \newline \textit{(0.02\%)} & 188 \newline \textit{(3.13\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}DDoS & 24 \newline \textit{(0.4\%)} & 37 \newline \textit{(0.62\%)} & 5927 \newline \cellcolor{tabhead}\textbf{(98.78\%)} & 0 \newline \textit{(0\%)} & 12 \newline \textit{(0.2\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}Port Scan & 20 \newline \textit{(0.33\%)} & 110 \newline \textit{(1.83\%)} & 4 \newline \textit{(0.07\%)} & 5848 \newline \cellcolor{tabhead}\textbf{(97.47\%)} & 18 \newline \textit{(0.3\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}FTP & 463 \newline \textit{(7.72\%)} & 862 \newline \textit{(14.37\%)} & 0 \newline \textit{(0\%)} & 0 \newline \textit{(0\%)} & 4675 \newline \cellcolor{tabhead}\textbf{(77.92\%)} & \\ \hline
    \end{tabular}

    \label{tab:cicids2-heartbleed-one-shot}
\end{table}


\begin{table}[H]
    \caption{CICIDS2017 One-Shot Accuracy (Heartbleed not in Training) Using Different $j$ Votes}
    \centering
       \begin{tabular}{|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|}
        \hline
        \rowcolor{tabhead}
         No Votes & Overall & \multicolumn{2}{c|}{New Class (Heartbleed)} &  \multicolumn{2}{c|}{Normal} \\ \cline{3-6} 
        \rowcolor{tabhead}
        ($j$) & Accuracy&  TPR & FNR & TNR & FPR \\  \hline
        \cellcolor{tabhead}1&77.03\% &56.42\% &31.93\% &63.37\% &36.63\%\\ \hline
        \cellcolor{tabhead}5&82.7\% &64.88\% &31.97\% &74.45\% &25.55\%\\ \hline
        \cellcolor{tabhead}10&84.19\% &70.25\% &27.07\% &76.03\% &23.97\%\\ \hline
        \cellcolor{tabhead}15&84.97\% &74.42\% &23.1\% &75.78\% &24.22\%\\ \hline
        \cellcolor{tabhead}20&85.32\% &76.35\% &21.27\% &75.62\% &24.38\%\\ \hline
        \cellcolor{tabhead}25&85.56\% &77.63\% &19.98\% &75.53\% &24.47\%\\ \hline
        \cellcolor{tabhead}30&85.77\% &78.6\% &19.02\% &75.62\% &24.38\%\\ \hline

     \hline 

    \end{tabular}
    
    \label{tab:cicids2-heartbleed-one-shot-pairs}
    
\end{table}


==> result-tables/one-shot/cicids2_portscan.tex <==
\begin{table}[h]
    \centering
    \caption{CICIDS2017 One-Shot Confusion Matrix (Port Scan Not in Training)}
    \begin{tabular}{|C{0.15\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\columnwidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.125\NetTableWidth}|C{0.1\NetTableWidth}|}
    \hhline{~-----~}
    \multicolumn{1}{c|}{} &
    \multicolumn{5}{c|}{\cellcolor{tabhead}Predicted Class} & \multicolumn{1}{|c}{}  \\
    \hline
    \rowcolor{tabhead}
     Correct &  Normal & Heart-bleed & DDoS & Port Scan & FTP & Overall \\ \hline
    \cellcolor{tabhead}Normal & 5091 \newline \cellcolor{tabhead}\textbf{(84.85\%)} & 529 \newline \textit{(8.82\%)} & 21 \newline \textit{(0.35\%)} & 334 \newline \textit{(5.57\%)} & 25 \newline \textit{(0.42\%)} & \multirow{5}{*}{80.68\%}\\ \cline{1-6}
    \cellcolor{tabhead}Heartbleed & 1324 \newline \textit{(22.07\%)} & 3669 \newline \cellcolor{tabhead}\textbf{(61.15\%)} & 0 \newline \textit{(0\%)} & 866 \newline \textit{(14.43\%)} & 141 \newline \textit{(2.35\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}DDoS & 16 \newline \textit{(0.27\%)} & 47 \newline \textit{(0.78\%)} & 5882 \newline \cellcolor{tabhead}\textbf{(98.03\%)} & 35 \newline \textit{(0.58\%)} & 20 \newline \textit{(0.33\%)} & \\ \cline{1-6}
    \cellcolor{classcol}Port Scan & 76 \newline \textit{(1.27\%)} & 639 \newline \textit{(10.65\%)} & 4 \newline \textit{(0.07\%)} & 5190 \newline \cellcolor{classcol}\textbf{(86.5\%)} & 91 \newline \textit{(1.52\%)} & \\ \cline{1-6}
    \cellcolor{tabhead}FTP & 362 \newline \textit{(6.03\%)} & 768 \newline \textit{(12.8\%)} & 0 \newline \textit{(0\%)} & 499 \newline \textit{(8.32\%)} & 4371 \newline \cellcolor{tabhead}\textbf{(72.85\%)} & \\ \hline
    \end{tabular}

    \label{tab:cicids2-portscan-one-shot}
\end{table}


\begin{table}[H]
    \caption{CICIDS2017 One-Shot Accuracy (Port Scan not in Training) Using Different $j$ Votes}
    \centering
       \begin{tabular}{|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|C{0.16\NetTableWidth}|}
        \hline
        \rowcolor{tabhead}
         No Votes & Overall & \multicolumn{2}{c|}{New Class (Port Scan)} &  \multicolumn{2}{c|}{Normal} \\ \cline{3-6} 
        \rowcolor{tabhead}
        ($j$) & Accuracy&  TPR & FNR & TNR & FPR \\  \hline
    
        \cellcolor{tabhead}1&70.41\% &74.58\% &3.95\% &69.92\% &30.08\%\\ \hline
        \cellcolor{tabhead}5&80.68\% &86.5\% &1.27\% &84.85\% &15.15\%\\ \hline
        \cellcolor{tabhead}10&82.08\% &87.32\% &0.72\% &85.6\% &14.4\%\\ \hline
        \cellcolor{tabhead}15&82.62\% &87.2\% &0.68\% &85.68\% &14.32\%\\ \hline
        \cellcolor{tabhead}20&82.7\% &87.05\% &0.7\% &85.88\% &14.12\%\\ \hline
        \cellcolor{tabhead}25&82.73\% &86.9\% &0.67\% &85.68\% &14.32\%\\ \hline
        \cellcolor{tabhead}30&82.69\% &86.73\% &0.67\% &85.6\% &14.4\%\\ \hline

     \hline 

    \end{tabular}
    
    \label{tab:cicids2-portscan-one-shot-pairs}
    
\end{table}

